Mid-Infrared Atomic Fine-Structure Emission Line Spectra of Luminous Infrared Galaxies: Spitzer/IRS Spectra of the GOALS Sample

We present the data and our analysis of MIR fine-structure emission lines detected in Spitzer/IRS high-res spectra of 202 local LIRGs observed as part of the GOALS project. We detect emission lines of [SIV], [NeII], [NeV], [NeIII], [SIII]18.7, [OIV], [FeII], [SIII]33.5, and [SiII]. Over 75% of our galaxies are classified as starburst (SB) sources in the MIR. We compare ratios of the emission line fluxes to stellar photo- and shock-ionization models to constrain the gas properties in the SB nuclei. Comparing the [SIV]/[NeII] and [NeIII]/[NeII] ratios to the Starburst99-Mappings III models with an instantaneous burst history, the line ratios suggest that the SB in our LIRGs have ages of 1-4.5Myr, metallicities of 1-2Z_sun, and ionization parameters of 2-8e7cm/s. Based on the [SIII]/[SIII] ratios, the electron density in LIRG nuclei has a median electron density of ~300cm-3 for sources above the low density limit. We also find that strong shocks are likely present in 10 SB sources. A significant fraction of the GOALS sources have resolved neon lines and 5 show velocity differences of >200km/s in [NeIII] or [NeV] relative to [NeII]. Furthermore, 6 SB and 5 AGN LIRGs show a trend of increasing line width with ionization potential, suggesting the possibility of a compact energy source and stratified ISM in their nuclei. We confirm a strong correlation between the [NeII]+[NeIII] emission, as well as [SIII]33.5, with both the IR luminosity and the 24um warm dust emission measured from the spectra. Finally, we find no correlation between the hardness of the radiation field or the line width and the ratio of the total IR to 8um emission (IR8). This may be because the IR luminosity and the MIR fine-structure lines are sensitive to different timescales over the SB, or that IR8 is more sensitive to the geometry of the warm dust region than the radiation field producing the HII region emission.

==> Metadata <==

Mid-Infrared Atomic Fine-Structure Emission Line Spectra of Luminous Infrared Galaxies: Spitzer/IRS Spectra of the GOALS Sample

H. Inami (1,2), L. Armus (2), V. Charmandaris (3,4,5), B. Groves (6), L. Kewley (7), A. Petric (8), S. Stierwalt (9,2), T. D\'iaz-Santos (2), J. Surace (2), J. Rich (10), S. Haan (11), J. Howell (2), A. Evans (9,12), J. Mazzarella (13), J. Marshall (2), P. Appleton (14), S. Lord (13), H. Spoon (15), D. Frayer (12), H. Matsuhara (16), S. Veilleux (17)    ( (1) NOAO, (2) SSC/Caltech, (3) University of Crete, (4) IESL/Foundation for Research & Technology-Hellas, (5) Observatoire de Paris, (6) MPIA, (7) The Australian National University, (8) Caltech, (9) University of Virginia, (10) The Carnegie Observatories, (11) CSIRO, (12) NRAO, (13) IPAC, (14) NASA Herschel Science Center, (15) Cornell University, (16) JAXA/ISAS, (17) University of Maryland )


We present the data and our analysis of MIR fine-structure emission lines detected in Spitzer/IRS high-resolution spectra of 202 local LIRGs observed as part of the GOALS project.  We detect emission lines of [SIV], [NeII], [NeV], [NeIII], [SIII]18.7, [OIV], [FeII], [SIII]33.5, and [SiII]. More than 75% of our sample are classified as starburst (SB) dominated sources in the MIR, based on the [NeV]/[NeII] ratios and EQW of the 6.2um PAH feature.  We compare ratios of the emission line fluxes to predictions from stellar photo-ionization and shock-ionization models to constrain the physical and chemical properties of the gas in the SB nuclei.  Comparing the [SIV]/[NeII] and [NeIII]/[NeII] line ratios to the Starburst99-Mappings III models with an instantaneous burst history, the emission line ratios suggest that the nuclear SB in our LIRGs have ages of 1-4.5 Myr, metallicities of 1-2 Z_sun, and ionization parameters of 2-8 x 10^7 cm/s.  Based on the [SIII]/[SIII] ratios, the electron density in LIRG nuclei is typically one to a few hundred cm-3 with a median electron density of ~300 cm-3, for those sources above the low density limit for these lines.  We also find that strong shocks are likely present in 10 SB dominated sources.  A significant fraction of the GOALS sources (80) have resolved neon emission lines and 5 show velocity differences of > 200 km/s in [NeIII] or [NeV] relative to [NeII].  Furthermore, 6 SB and 5 AGN dominated LIRGs show a clear trend of increasing line width with ionization potential, suggesting the possibility of a compact energy source and stratified ISM in their nuclei.  We confirm a strong correlation between the [NeII] + [NeIII] emission, as well as [SIII]33.5, with both the IR luminosity and the 24um warm dust emission measured from the spectra, consistent with all three lines tracing ongoing star formation.  Finally, we find no correlation between the hardness of the radiation field or the emission line width and the ratio of the total IR to 8um emission (IR8).  This may be a function of the fact that the IR luminosity and the MIR fine-structure lines are sensitive to different timescales over the SB, or that IR8 is more sensitive to the geometry of the warm dust region than the radiation field producing the HII region emission.

